Safely Learning Dynamical Systems

A fundamental challenge in learning an unknown dynamical system is to reduce model uncertainty by making measurements while maintaining safety. We formulate a mathematical definition of what it means to safely learn a dynamical system by sequentially deciding where to initialize trajectories. The state of the system must stay within a safety region for a horizon of $T$ time steps under the action of all dynamical systems that (i) belong to a given initial uncertainty set, and (ii) are consistent with information gathered so far. First, we consider safely learning a linear dynamical system involving $n$ states. For the case $T=1$, we present an LP-based algorithm that either safely recovers the true dynamics from at most $n$ trajectories, or certifies that safe learning is impossible. For $T=2$, we give an SDP representation of the set of safe initial conditions and show that $\lceil n/2 \rceil$ trajectories generically suffice for safe learning. For $T = \infty$, we provide SDP-representable inner approximations of the set of safe initial conditions and show that one trajectory generically suffices for safe learning. We extend a number of our results to the cases where the initial uncertainty set contains sparse, low-rank, or permutation matrices, or when the system has a control input. Second, we consider safely learning a general class of nonlinear dynamical systems. For the case $T=1$, we give an SOCP-based representation of the set of safe initial conditions. For $T=\infty$, we provide semidefinite representable inner approximations to the set of safe initial conditions. We show how one can safely collect trajectories and fit a polynomial model of the nonlinear dynamics that is consistent with the initial uncertainty set and best agrees with the observations. We also present some extensions to cases where the measurements are noisy or the dynamical system involves disturbances.

==> olderfiles/conclusion.tex <==
\section{Conclusion}
Concluding remarks and maybe next steps.

==> problem_formulation.tex <==
\section{Problem Formulation}
We consider a discrete-time dynamical system
\begin{equation}\label{eq:dynamics}
x_{k+1} = f(x_k),
\end{equation}
where $x\in \R^n$ is the state of the system and $f: \R^n \rightarrow \R^n$ is an unknown map that we would like to learn by making queries to the system.
% We examine a dynamical system with state variable $x \in \R^n$.
% We have a discrete time dynamics defined by a function $f: \R^n \rightarrow \R^n$.
% Thus the state evolves like so:
We consider a setting where we are given as input a set $S \subset \R^n$, called the \emph{safety region}, in which the state should remain throughout the learning process. More precisely, in order to learn $f$, we are only allowed to query points that are in $S$ and that remain in $S$ under the dynamics (\ref{eq:dynamics}) for a short time period. Obviously, if we know nothing about $f$, this task is impossible. We assume, therefore, that the dynamics $f$ belongs to a set of dynamics $U_f$, which we call the \emph{uncertainty set}. Our aim, in a sense, is to model the interplay between \emph{safety} and \emph{uncertainty} in learning dynamical systems. 



We define the \emph{safe learning problem} as the problem of learning the action of $f$ on $S$ via 


We are also interested in identifying conditions on $f$, $S$, $U_f$ under which we can safely learn $f$

the safe learning problem can be tractably solved using techniques from conic optimization.

***Motivate short time period
***Bring in out interest in classifying tractability /optimization viewpoint
*Objective function
*** One and two step safe...
*** Outline of contributions (linear 1 step 2 step, extension to nonlinear)
*** CT motivation of Vikas
***Characterizing safety region

** Define T step safety

**** Value of collecting information on the fly





Our trajectories must initiate within the safety region and should remain in the safety region under the dynamics of the system.
The (possibly repeated) action of $f$ to the point that we query should also 
We do not know the function $f$, but we may assume it belongs to a set of dynamics; i.e. $f \in U_f$.
% One special case we investigate is linear dynamics, i.e. when $f(x) = A x$ for some $A \in \R^{n \times n}$.
% Here we may assume that $A$ belongs to a set of matrices; i.e. $A \in U_A \subset \R^{n \times n}$.

We refer to points in the safety region as \emph{safe}.
The broad problem we approach in this paper is to learn the dynamics safely.
More precisely, we would like to learn $f$ in a way such that the state variable never leaves the safety region.
We can consider choosing an $x_0$ and then observing a \emph{trajectory} of length $t$, i.e. $\left \{ x_k \mid k = 1, \dots ,t \right \}$.
Each trajectory gives information on the dynamics.
Of course, to maintain safety we must ensure that $x_0$ is safe and that $x_k$ remains safe.
We say a point $x$ is \emph{one-step safe} if $x \in S$ and $f(x) \in S$.
We say a point $x$ is \emph{two-step safe} if $x \in S$ and $f(x) \in S$ and $f(f(x)) \in S$.
In certain cases, we can characterize how many trajectories we need to exactly learn the dynamics $f$.
We may also consider a cost of learning, i.e. there may be a cost to starting a trajectory at a certain point.
In this case we wish to learn the dynamics not only safely, but also with minimum cost.
